Embedding products of graphs into Euclidean spaces

For any collection of graphs we find the minimal dimension d such that the product of these graphs is embeddable into the d-dimensional Euclidean space. In particular, we prove that the n-th powers of the Kuratowsky graphs are not embeddable into the 2n-dimensional Euclidean space. This is a solution of a problem of Menger from 1929. The idea of the proof is the reduction to a problem from so-called Ramsey link theory: we show that any embedding of L into the (2n-1)-dimensional sphere, where L is the join of n copies of a 4-point set, has a pair of linked (n-1)-dimensional spheres.

==> FIG2.TEX <==
%LaTeX representation of Charton picture (version 1.96)
%Copyright (c) S.Trifonov, D.Tejblum, 1993-4
%FILE: C:\USER\MISHA\FIG2.tex
%DATE: Sun Oct 12 21:01:59 2003
%------------
\setlength{\unitlength}{0.075in}
\begin{picture}(26.63,24.85)
\put(16.76,3.33){{\setbox0=\hbox{$K_{4,4}$}\lower\ht0\box0}}
\put(13.43,19.83){{\setbox0=\hbox{$R^3$}\lower\ht0\box0}}
\put(26.63,16.66){{\setbox0=\hbox{$R^1$}\lower\ht0\box0}}
\put(1.56,24.83){{\setbox0=\hbox{$R^1$}\lower\ht0\box0}}
\special{em:linewidth 0.014in}
\put(0.10,10.00){\special{em:moveto}}
\put(8.10,1.66){\special{em:lineto}}
\put(0.06,5.00){\special{em:moveto}}
\put(8.26,1.66){\special{em:lineto}}
\put(0.23,5.00){{\setbox0=\hbox{$\scriptstyle\bullet$}\kern-.4\wd0\lower.5\ht0\box0}}
\put(3.56,5.80){\special{em:moveto}}
\put(0.00,5.16){\special{em:lineto}}
\put(5.16,6.06){\special{em:moveto}}
\put(4.56,6.00){\special{em:lineto}}
\put(8.13,6.63){\special{em:moveto}}
\put(6.60,6.33){\special{em:lineto}}
\put(10.26,7.00){\special{em:moveto}}
\put(9.20,6.83){\special{em:lineto}}
\put(18.30,8.53){\special{em:moveto}}
\put(11.83,7.30){\special{em:lineto}}
\put(16.86,9.93){\special{em:moveto}}
\put(23.76,11.83){\special{em:lineto}}
\put(15.96,9.66){\special{em:moveto}}
\put(16.00,9.66){\special{em:lineto}}
\put(14.20,9.13){\special{em:moveto}}
\put(15.06,9.40){\special{em:lineto}}
\put(11.10,8.23){\special{em:moveto}}
\put(12.93,8.76){\special{em:lineto}}
\put(10.00,7.96){\special{em:moveto}}
\put(10.40,8.03){\special{em:lineto}}
\put(7.93,7.36){\special{em:moveto}}
\put(9.26,7.76){\special{em:lineto}}
\put(6.36,6.93){\special{em:moveto}}
\put(6.93,7.13){\special{em:lineto}}
\put(4.26,6.33){\special{em:moveto}}
\put(4.63,6.50){\special{em:lineto}}
\put(0.03,5.20){\special{em:moveto}}
\put(3.56,6.16){\special{em:lineto}}
\put(7.26,5.00){\special{em:moveto}}
\put(13.46,5.00){\special{em:lineto}}
\put(5.43,5.00){\special{em:moveto}}
\put(5.90,5.00){\special{em:lineto}}
\put(5.46,5.00){\special{em:moveto}}
\put(5.73,5.00){\special{em:lineto}}
\put(0.06,5.03){\special{em:moveto}}
\put(4.66,5.03){\special{em:lineto}}
\put(6.03,7.76){\special{em:moveto}}
\put(13.43,4.96){\special{em:lineto}}
\put(4.50,8.40){\special{em:moveto}}
\put(5.03,8.13){\special{em:lineto}}
\put(0.06,10.00){\special{em:moveto}}
\put(3.53,8.73){\special{em:lineto}}
\put(2.66,9.76){\special{em:moveto}}
\put(0.10,10.00){\special{em:lineto}}
\put(4.26,9.66){\special{em:moveto}}
\put(3.80,9.70){\special{em:lineto}}
\put(7.13,9.43){\special{em:moveto}}
\put(5.00,9.60){\special{em:lineto}}
\put(9.20,9.26){\special{em:moveto}}
\put(8.03,9.36){\special{em:lineto}}
\put(18.33,8.53){\special{em:moveto}}
\put(10.03,9.20){\special{em:lineto}}
\put(15.03,11.16){\special{em:moveto}}
\put(23.56,11.83){\special{em:lineto}}
\put(12.43,10.96){\special{em:moveto}}
\put(13.86,11.06){\special{em:lineto}}
\put(8.96,10.66){\special{em:moveto}}
\put(11.00,10.83){\special{em:lineto}}
\put(6.76,10.50){\special{em:moveto}}
\put(7.96,10.63){\special{em:lineto}}
\put(4.86,10.33){\special{em:moveto}}
\put(5.63,10.43){\special{em:lineto}}
\put(3.56,10.26){\special{em:moveto}}
\put(4.03,10.26){\special{em:lineto}}
\put(0.06,10.00){\special{em:moveto}}
\put(2.73,10.20){\special{em:lineto}}
\put(0.23,15.00){\special{em:moveto}}
\put(8.23,1.50){\special{em:lineto}}
\put(10.96,6.90){\special{em:moveto}}
\put(13.43,5.00){\special{em:lineto}}
\put(3.96,12.13){\special{em:moveto}}
\put(10.96,6.86){\special{em:lineto}}
\put(0.10,15.03){\special{em:moveto}}
\put(3.00,12.86){\special{em:lineto}}
\put(7.20,12.46){\special{em:moveto}}
\put(18.36,8.53){\special{em:lineto}}
\put(7.16,12.46){\special{em:moveto}}
\put(11.23,11.06){\special{em:lineto}}
\put(3.23,13.90){\special{em:moveto}}
\put(6.03,12.90){\special{em:lineto}}
\put(0.13,15.00){\special{em:moveto}}
\put(2.26,14.23){\special{em:lineto}}
\put(11.20,13.50){\special{em:moveto}}
\put(23.66,11.80){\special{em:lineto}}
\put(5.70,14.23){\special{em:moveto}}
\put(9.73,13.70){\special{em:lineto}}
\put(2.93,14.63){\special{em:moveto}}
\put(4.73,14.36){\special{em:lineto}}
\put(0.06,15.03){\special{em:moveto}}
\put(2.10,14.73){\special{em:lineto}}
\put(18.36,8.50){\special{em:moveto}}
\put(0.10,20.16){\special{em:lineto}}
\put(23.56,11.83){\special{em:lineto}}
\put(8.23,1.66){\special{em:moveto}}
\put(0.10,20.00){\special{em:lineto}}
\put(13.43,5.00){\special{em:lineto}}
\put(5.96,0.00){\special{em:moveto}}
\put(25.96,13.33){\special{em:lineto}}
\put(0.10,21.66){\special{em:moveto}}
\put(0.10,3.16){\special{em:lineto}}
\put(23.56,11.83){{\setbox0=\hbox{$\scriptstyle\bullet$}\kern-.4\wd0\lower.5\ht0\box0}}
\put(18.36,8.50){{\setbox0=\hbox{$\scriptstyle\bullet$}\kern-.4\wd0\lower.5\ht0\box0}}
\put(13.43,5.00){{\setbox0=\hbox{$\scriptstyle\bullet$}\kern-.4\wd0\lower.5\ht0\box0}}
\put(8.23,1.66){{\setbox0=\hbox{$\scriptstyle\bullet$}\kern-.4\wd0\lower.5\ht0\box0}}
\put(0.10,10.00){{\setbox0=\hbox{$\scriptstyle\bullet$}\kern-.4\wd0\lower.5\ht0\box0}}
\put(0.10,15.00){{\setbox0=\hbox{$\scriptstyle\bullet$}\kern-.4\wd0\lower.5\ht0\box0}}
\put(0.10,20.00){{\setbox0=\hbox{$\scriptstyle\bullet$}\kern-.4\wd0\lower.5\ht0\box0}}
\end{picture}


==> fig1.TEX <==
%LaTeX representation of Charton picture (version 1.96)
%Copyright (c) S.Trifonov, D.Tejblum, 1993-4
%FILE: C:\USER\MISHA\FIG1.tex
%DATE: Sun Oct 12 19:44:32 2003
%------------
\setlength{\unitlength}{0.075in}
\begin{picture}(51.90,22.18)

\put(25.21,11.66){{\setbox0=\hbox{$\to$}\lower\ht0\box0}}
\put(40.15,0.00){{\setbox0=\hbox{$K_{3,3}$}\lower\ht0\box0}}
\put(45.08,10.00){{\setbox0=\hbox{$\scriptstyle\bullet$}\kern-.4\wd0\lower.5\ht0\box0}}
\put(35.08,10.00){{\setbox0=\hbox{$\scriptstyle\bullet$}\kern-.4\wd0\lower.5\ht0\box0}}
\special{em:linewidth 0.014in}
\put(34.95,10.00){\special{em:moveto}}
\put(45.35,10.00){\special{em:lineto}}
\put(48.55,16.66){\special{em:moveto}}
\put(45.21,10.00){\special{em:lineto}}
\put(48.28,3.33){\special{em:lineto}}
\put(31.88,16.66){\special{em:moveto}}
\put(35.21,10.00){\special{em:lineto}}
\put(31.75,3.33){\special{em:lineto}}
\put(31.75,3.33){\special{em:moveto}}
\put(30.73,4.41){\special{em:lineto}}
\put(29.95,5.50){\special{em:lineto}}
\put(29.35,6.58){\special{em:lineto}}
\put(28.76,8.01){\special{em:lineto}}
\put(28.41,9.45){\special{em:lineto}}
\put(28.26,10.88){\special{em:lineto}}
\put(28.26,11.28){\special{em:lineto}}
\put(28.36,12.75){\special{em:lineto}}
\put(28.66,14.21){\special{em:lineto}}
\put(29.20,15.68){\special{em:lineto}}
\put(29.76,16.78){\special{em:lineto}}
\put(30.51,17.88){\special{em:lineto}}
\put(31.50,18.98){\special{em:lineto}}
\put(32.45,19.81){\special{em:lineto}}
\put(33.70,20.65){\special{em:lineto}}
\put(35.00,21.28){\special{em:lineto}}
\put(36.48,21.76){\special{em:lineto}}
\put(37.65,21.98){\special{em:lineto}}
\put(38.30,22.05){\special{em:lineto}}
\put(39.05,22.06){\special{em:lineto}}
\put(40.58,21.96){\special{em:lineto}}
\put(41.93,21.68){\special{em:lineto}}
\put(43.30,21.20){\special{em:lineto}}
\put(44.55,20.56){\special{em:lineto}}
\put(45.75,19.73){\special{em:lineto}}
\put(46.68,18.90){\special{em:lineto}}
\put(47.43,18.06){\special{em:lineto}}
\put(48.05,17.23){\special{em:lineto}}
\put(48.41,16.66){\special{em:lineto}}
\put(31.88,16.66){\special{em:moveto}}
\put(32.51,17.66){\special{em:lineto}}
\put(33.63,19.00){\special{em:lineto}}
\put(34.76,20.00){\special{em:lineto}}
\put(35.90,20.75){\special{em:lineto}}
\put(37.03,21.31){\special{em:lineto}}
\put(38.23,21.75){\special{em:lineto}}
\put(39.78,22.08){\special{em:lineto}}
\put(40.40,22.15){\special{em:lineto}}
\put(41.23,22.16){\special{em:lineto}}
\put(42.55,22.10){\special{em:lineto}}
\put(43.73,21.88){\special{em:lineto}}
\put(44.93,21.51){\special{em:lineto}}
\put(46.05,21.03){\special{em:lineto}}
\put(47.41,20.20){\special{em:lineto}}
\put(48.45,19.36){\special{em:lineto}}
\put(49.26,18.53){\special{em:lineto}}
\put(50.10,17.43){\special{em:lineto}}
\put(50.61,16.60){\special{em:lineto}}
\put(51.13,15.50){\special{em:lineto}}
\put(51.50,14.40){\special{em:lineto}}
\put(51.70,13.56){\special{em:lineto}}
\put(51.86,12.46){\special{em:lineto}}
\put(51.90,11.50){\special{em:lineto}}
\put(51.85,10.40){\special{em:lineto}}
\put(51.68,9.30){\special{em:lineto}}
\put(51.38,8.20){\special{em:lineto}}
\put(50.96,7.10){\special{em:lineto}}
\put(50.38,6.00){\special{em:lineto}}
\put(49.61,4.90){\special{em:lineto}}
\put(48.90,4.06){\special{em:lineto}}
\put(48.15,3.33){\special{em:lineto}}
\put(46.95,16.66){\special{em:moveto}}
\put(47.08,16.66){\special{em:lineto}}
\put(47.35,16.66){\special{em:lineto}}
\put(31.75,3.33){{\setbox0=\hbox{$\scriptstyle\bullet$}\kern-.4\wd0\lower.5\ht0\box0}}
\put(48.28,3.33){{\setbox0=\hbox{$\scriptstyle\bullet$}\kern-.4\wd0\lower.5\ht0\box0}}
\put(48.55,16.66){{\setbox0=\hbox{$\scriptstyle\bullet$}\kern-.4\wd0\lower.5\ht0\box0}}
\put(31.75,16.66){{\setbox0=\hbox{$\scriptstyle\bullet$}\kern-.4\wd0\lower.5\ht0\box0}}
\put(31.75,3.33){\special{em:moveto}}
\put(48.15,3.33){\special{em:lineto}}
\put(31.75,16.66){\special{em:moveto}}
\put(48.28,16.66){\special{em:lineto}}
\put(11.88,0.16){{\setbox0=\hbox{$K_5$}\lower\ht0\box0}}
\put(3.48,3.33){\special{em:moveto}}
\put(2.70,4.15){\special{em:lineto}}
\put(2.18,4.76){\special{em:lineto}}
\put(1.46,5.85){\special{em:lineto}}
\put(0.91,6.93){\special{em:lineto}}
\put(0.51,8.01){\special{em:lineto}}
\put(0.28,8.83){\special{em:lineto}}
\put(0.05,10.26){\special{em:lineto}}
\put(0.00,11.28){\special{em:lineto}}
\put(0.10,12.75){\special{em:lineto}}
\put(0.31,13.85){\special{em:lineto}}
\put(0.65,14.95){\special{em:lineto}}
\put(1.11,16.05){\special{em:lineto}}
\put(1.73,17.15){\special{em:lineto}}
\put(2.55,18.25){\special{em:lineto}}
\put(3.61,19.35){\special{em:lineto}}
\put(4.68,20.18){\special{em:lineto}}
\put(6.11,21.01){\special{em:lineto}}
\put(7.30,21.50){\special{em:lineto}}
\put(8.63,21.86){\special{em:lineto}}
\put(9.71,22.03){\special{em:lineto}}
\put(10.80,22.08){\special{em:lineto}}
\put(12.28,21.98){\special{em:lineto}}
\put(13.66,21.70){\special{em:lineto}}
\put(15.05,21.21){\special{em:lineto}}
\put(16.28,20.58){\special{em:lineto}}
\put(17.50,19.75){\special{em:lineto}}
\put(18.70,18.65){\special{em:lineto}}
\put(19.85,17.18){\special{em:lineto}}
\put(20.15,16.66){\special{em:lineto}}
\put(3.61,16.66){\special{em:moveto}}
\put(4.25,17.66){\special{em:lineto}}
\put(5.05,18.66){\special{em:lineto}}
\put(6.08,19.66){\special{em:lineto}}
\put(7.08,20.41){\special{em:lineto}}
\put(8.05,20.98){\special{em:lineto}}
\put(9.33,21.55){\special{em:lineto}}
\put(10.86,21.98){\special{em:lineto}}
\put(11.81,22.13){\special{em:lineto}}
\put(12.98,22.18){\special{em:lineto}}
\put(14.53,22.08){\special{em:lineto}}
\put(15.86,21.80){\special{em:lineto}}
\put(17.21,21.31){\special{em:lineto}}
\put(18.46,20.68){\special{em:lineto}}
\put(19.66,19.85){\special{em:lineto}}
\put(20.58,19.01){\special{em:lineto}}
\put(21.53,17.91){\special{em:lineto}}
\put(22.25,16.81){\special{em:lineto}}
\put(22.80,15.71){\special{em:lineto}}
\put(23.20,14.61){\special{em:lineto}}
\put(23.55,13.15){\special{em:lineto}}
\put(23.66,11.50){\special{em:lineto}}
\put(23.61,10.40){\special{em:lineto}}
\put(23.36,8.93){\special{em:lineto}}
\put(22.88,7.46){\special{em:lineto}}
\put(22.36,6.36){\special{em:lineto}}
\put(21.66,5.26){\special{em:lineto}}
\put(20.76,4.16){\special{em:lineto}}
\put(19.88,3.33){\special{em:lineto}}
\put(20.28,16.66){\special{em:moveto}}
\put(18.55,10.16){\special{em:lineto}}
\put(20.01,3.33){\special{em:lineto}}
\put(11.88,10.00){\special{em:moveto}}
\put(16.81,8.33){\special{em:lineto}}
\put(19.88,3.33){\special{em:lineto}}
\put(20.28,16.66){\special{em:moveto}}
\put(16.81,11.66){\special{em:lineto}}
\put(11.88,10.00){\special{em:lineto}}
\put(18.68,16.66){\special{em:moveto}}
\put(18.81,16.66){\special{em:lineto}}
\put(19.08,16.66){\special{em:lineto}}
\put(3.48,16.83){\special{em:moveto}}
\put(5.21,10.00){\special{em:lineto}}
\put(3.48,3.33){\special{em:lineto}}
\put(3.48,3.33){\special{em:moveto}}
\put(6.95,8.50){\special{em:lineto}}
\put(11.88,10.16){\special{em:lineto}}
\put(3.48,16.66){\special{em:moveto}}
\put(6.81,11.50){\special{em:lineto}}
\put(11.88,10.00){\special{em:lineto}}
\put(11.88,10.00){{\setbox0=\hbox{$\scriptstyle\bullet$}\kern-.4\wd0\lower.5\ht0\box0}}
\put(3.48,3.33){{\setbox0=\hbox{$\scriptstyle\bullet$}\kern-.4\wd0\lower.5\ht0\box0}}
\put(20.01,3.33){{\setbox0=\hbox{$\scriptstyle\bullet$}\kern-.4\wd0\lower.5\ht0\box0}}
\put(20.28,16.66){{\setbox0=\hbox{$\scriptstyle\bullet$}\kern-.4\wd0\lower.5\ht0\box0}}
\put(3.48,16.66){{\setbox0=\hbox{$\scriptstyle\bullet$}\kern-.4\wd0\lower.5\ht0\box0}}
\put(3.48,3.33){\special{em:moveto}}
\put(20.01,3.33){\special{em:lineto}}
\put(3.48,16.66){\special{em:moveto}}
\put(20.15,16.66){\special{em:lineto}}
\end{picture}


==> fig1prime.TEX <==
%LaTeX representation of Charton picture (version 1.96)
%Copyright (c) S.Trifonov, D.Tejblum, 1993-4
%FILE: C:\USER\MISHA\FIG1.tex
%DATE: Sun Oct 12 19:44:32 2003
%------------
\setlength{\unitlength}{0.075in}
\begin{picture}(51.90,22.18)

%\put(25.21,11.66){{\setbox0=\hbox{$\to$}\lower\ht0\box0}}
\put(40.15,0.00){{\setbox0=\hbox{$K_{3,3}$}\lower\ht0\box0}}
\put(45.08,10.00){{\setbox0=\hbox{$\scriptstyle\bullet$}\kern-.4\wd0\lower.5\ht0\box0}}
\put(35.08,10.00){{\setbox0=\hbox{$\scriptstyle\bullet$}\kern-.4\wd0\lower.5\ht0\box0}}
\special{em:linewidth 0.014in}
\put(34.95,10.00){\special{em:moveto}}
\put(45.35,10.00){\special{em:lineto}}
\put(48.55,16.66){\special{em:moveto}}
\put(45.21,10.00){\special{em:lineto}}
\put(48.28,3.33){\special{em:lineto}}
\put(31.88,16.66){\special{em:moveto}}
\put(35.21,10.00){\special{em:lineto}}
\put(31.75,3.33){\special{em:lineto}}
\put(31.75,3.33){\special{em:moveto}}
\put(30.73,4.41){\special{em:lineto}}
\put(29.95,5.50){\special{em:lineto}}
\put(29.35,6.58){\special{em:lineto}}
\put(28.76,8.01){\special{em:lineto}}
\put(28.41,9.45){\special{em:lineto}}
\put(28.26,10.88){\special{em:lineto}}
\put(28.26,11.28){\special{em:lineto}}
\put(28.36,12.75){\special{em:lineto}}
\put(28.66,14.21){\special{em:lineto}}
\put(29.20,15.68){\special{em:lineto}}
\put(29.76,16.78){\special{em:lineto}}
\put(30.51,17.88){\special{em:lineto}}
\put(31.50,18.98){\special{em:lineto}}
\put(32.45,19.81){\special{em:lineto}}
\put(33.70,20.65){\special{em:lineto}}
\put(35.00,21.28){\special{em:lineto}}
\put(36.48,21.76){\special{em:lineto}}
\put(37.65,21.98){\special{em:lineto}}
\put(38.30,22.05){\special{em:lineto}}
\put(39.05,22.06){\special{em:lineto}}
\put(40.58,21.96){\special{em:lineto}}
\put(41.93,21.68){\special{em:lineto}}
\put(43.30,21.20){\special{em:lineto}}
\put(44.55,20.56){\special{em:lineto}}
\put(45.75,19.73){\special{em:lineto}}
\put(46.68,18.90){\special{em:lineto}}
\put(47.43,18.06){\special{em:lineto}}
\put(48.05,17.23){\special{em:lineto}}
\put(48.41,16.66){\special{em:lineto}}
\put(31.88,16.66){\special{em:moveto}}
\put(32.51,17.66){\special{em:lineto}}
\put(33.63,19.00){\special{em:lineto}}
\put(34.76,20.00){\special{em:lineto}}
\put(35.90,20.75){\special{em:lineto}}
\put(37.03,21.31){\special{em:lineto}}
\put(38.23,21.75){\special{em:lineto}}
\put(39.78,22.08){\special{em:lineto}}
\put(40.40,22.15){\special{em:lineto}}
\put(41.23,22.16){\special{em:lineto}}
\put(42.55,22.10){\special{em:lineto}}
\put(43.73,21.88){\special{em:lineto}}
\put(44.93,21.51){\special{em:lineto}}
\put(46.05,21.03){\special{em:lineto}}
\put(47.41,20.20){\special{em:lineto}}
\put(48.45,19.36){\special{em:lineto}}
\put(49.26,18.53){\special{em:lineto}}
\put(50.10,17.43){\special{em:lineto}}
\put(50.61,16.60){\special{em:lineto}}
\put(51.13,15.50){\special{em:lineto}}
\put(51.50,14.40){\special{em:lineto}}
\put(51.70,13.56){\special{em:lineto}}
\put(51.86,12.46){\special{em:lineto}}
\put(51.90,11.50){\special{em:lineto}}
\put(51.85,10.40){\special{em:lineto}}
\put(51.68,9.30){\special{em:lineto}}
\put(51.38,8.20){\special{em:lineto}}
\put(50.96,7.10){\special{em:lineto}}
\put(50.38,6.00){\special{em:lineto}}
\put(49.61,4.90){\special{em:lineto}}
\put(48.90,4.06){\special{em:lineto}}
\put(48.15,3.33){\special{em:lineto}}
\put(46.95,16.66){\special{em:moveto}}
\put(47.08,16.66){\special{em:lineto}}
\put(47.35,16.66){\special{em:lineto}}
\put(31.75,3.33){{\setbox0=\hbox{$\scriptstyle\bullet$}\kern-.4\wd0\lower.5\ht0\box0}}
\put(48.28,3.33){{\setbox0=\hbox{$\scriptstyle\bullet$}\kern-.4\wd0\lower.5\ht0\box0}}
\put(48.55,16.66){{\setbox0=\hbox{$\scriptstyle\bullet$}\kern-.4\wd0\lower.5\ht0\box0}}
\put(31.75,16.66){{\setbox0=\hbox{$\scriptstyle\bullet$}\kern-.4\wd0\lower.5\ht0\box0}}
\put(31.75,3.33){\special{em:moveto}}
\put(48.15,3.33){\special{em:lineto}}
\put(31.75,16.66){\special{em:moveto}}
\put(48.28,16.66){\special{em:lineto}}
\put(11.88,0.16){{\setbox0=\hbox{$K_5$}\lower\ht0\box0}}
\put(3.48,3.33){\special{em:moveto}}
\put(2.70,4.15){\special{em:lineto}}
\put(2.18,4.76){\special{em:lineto}}
\put(1.46,5.85){\special{em:lineto}}
\put(0.91,6.93){\special{em:lineto}}
\put(0.51,8.01){\special{em:lineto}}
\put(0.28,8.83){\special{em:lineto}}
\put(0.05,10.26){\special{em:lineto}}
\put(0.00,11.28){\special{em:lineto}}
\put(0.10,12.75){\special{em:lineto}}
\put(0.31,13.85){\special{em:lineto}}
\put(0.65,14.95){\special{em:lineto}}
\put(1.11,16.05){\special{em:lineto}}
\put(1.73,17.15){\special{em:lineto}}
\put(2.55,18.25){\special{em:lineto}}
\put(3.61,19.35){\special{em:lineto}}
\put(4.68,20.18){\special{em:lineto}}
\put(6.11,21.01){\special{em:lineto}}
\put(7.30,21.50){\special{em:lineto}}
\put(8.63,21.86){\special{em:lineto}}
\put(9.71,22.03){\special{em:lineto}}
\put(10.80,22.08){\special{em:lineto}}
\put(12.28,21.98){\special{em:lineto}}
\put(13.66,21.70){\special{em:lineto}}
\put(15.05,21.21){\special{em:lineto}}
\put(16.28,20.58){\special{em:lineto}}
\put(17.50,19.75){\special{em:lineto}}
\put(18.70,18.65){\special{em:lineto}}
\put(19.85,17.18){\special{em:lineto}}
\put(20.15,16.66){\special{em:lineto}}
\put(3.61,16.66){\special{em:moveto}}
\put(4.25,17.66){\special{em:lineto}}
\put(5.05,18.66){\special{em:lineto}}
\put(6.08,19.66){\special{em:lineto}}
\put(7.08,20.41){\special{em:lineto}}
\put(8.05,20.98){\special{em:lineto}}
\put(9.33,21.55){\special{em:lineto}}
\put(10.86,21.98){\special{em:lineto}}
\put(11.81,22.13){\special{em:lineto}}
\put(12.98,22.18){\special{em:lineto}}
\put(14.53,22.08){\special{em:lineto}}
\put(15.86,21.80){\special{em:lineto}}
\put(17.21,21.31){\special{em:lineto}}
\put(18.46,20.68){\special{em:lineto}}
\put(19.66,19.85){\special{em:lineto}}
\put(20.58,19.01){\special{em:lineto}}
\put(21.53,17.91){\special{em:lineto}}
\put(22.25,16.81){\special{em:lineto}}
\put(22.80,15.71){\special{em:lineto}}
\put(23.20,14.61){\special{em:lineto}}
\put(23.55,13.15){\special{em:lineto}}
\put(23.66,11.50){\special{em:lineto}}
\put(23.61,10.40){\special{em:lineto}}
\put(23.36,8.93){\special{em:lineto}}
\put(22.88,7.46){\special{em:lineto}}
\put(22.36,6.36){\special{em:lineto}}
\put(21.66,5.26){\special{em:lineto}}
\put(20.76,4.16){\special{em:lineto}}
\put(19.88,3.33){\special{em:lineto}}
\put(20.28,16.66){\special{em:moveto}}
\put(18.55,10.16){\special{em:lineto}}
\put(20.01,3.33){\special{em:lineto}}
\put(11.88,10.00){\special{em:moveto}}
\put(16.81,8.33){\special{em:lineto}}
\put(19.88,3.33){\special{em:lineto}}
\put(20.28,16.66){\special{em:moveto}}
\put(16.81,11.66){\special{em:lineto}}
\put(11.88,10.00){\special{em:lineto}}
\put(18.68,16.66){\special{em:moveto}}
\put(18.81,16.66){\special{em:lineto}}
\put(19.08,16.66){\special{em:lineto}}
\put(3.48,16.83){\special{em:moveto}}
\put(5.21,10.00){\special{em:lineto}}
\put(3.48,3.33){\special{em:lineto}}
\put(3.48,3.33){\special{em:moveto}}
\put(6.95,8.50){\special{em:lineto}}
\put(11.88,10.16){\special{em:lineto}}
\put(3.48,16.66){\special{em:moveto}}
\put(6.81,11.50){\special{em:lineto}}
\put(11.88,10.00){\special{em:lineto}}
\put(11.88,10.00){{\setbox0=\hbox{$\scriptstyle\bullet$}\kern-.4\wd0\lower.5\ht0\box0}}
\put(3.48,3.33){{\setbox0=\hbox{$\scriptstyle\bullet$}\kern-.4\wd0\lower.5\ht0\box0}}
\put(20.01,3.33){{\setbox0=\hbox{$\scriptstyle\bullet$}\kern-.4\wd0\lower.5\ht0\box0}}
\put(20.28,16.66){{\setbox0=\hbox{$\scriptstyle\bullet$}\kern-.4\wd0\lower.5\ht0\box0}}
\put(3.48,16.66){{\setbox0=\hbox{$\scriptstyle\bullet$}\kern-.4\wd0\lower.5\ht0\box0}}
\put(3.48,3.33){\special{em:moveto}}
\put(20.01,3.33){\special{em:lineto}}
\put(3.48,16.66){\special{em:moveto}}
\put(20.15,16.66){\special{em:lineto}}
\end{picture}

